Large Scale Real-time Ridesharing with Service Guarantee on Road Networks

The mean occupancy rates of personal vehicle trips in the United States is only 1.6 persons per vehicle mile. Urban traffic gridlock is a familiar scene. Ridesharing has the potential to solve many environmental, congestion, and energy problems. In this paper, we introduce the problem of large scale real-time ridesharing with service guarantee on road networks. Servers and trip requests are dynamically matched while waiting time and service time constraints of trips are satisfied. We first propose two basic algorithms: a branch-and-bound algorithm and an integer programing algorithm. However, these algorithm structures do not adapt well to the dynamic nature of the ridesharing problem. Thus, we then propose a kinetic tree algorithm capable of better scheduling dynamic requests and adjusting routes on-the-fly. We perform experiments on a large real taxi dataset from Shanghai. The results show that the kinetic tree algorithm is faster than other algorithms in response time.

==> Preliminary.tex <==
\section{Preliminary: Optimal Tree Cover and Scalability Bottleneck}
\label{preliminary}

To proceed, let us first revisit how to discover the optimal tree for compressing the transitive closure~\cite{SIGMOD:AgrawalBJ:1989}, which contains three key steps: 
1) for each vertex, we compute all its predecessors $pred(v)$, which contains all the vertices which can reach $v$ (including itself). This is essentially the classical fast transitive closure computation, which compute the predecessor sets of each vertex iteratively following the topological order~\cite{SIGMOD:AgrawalBJ:1989}; 
2) for each edge $e=(v^\prime,v)$, we assign an edge weight, which is the size of $v$'s predecessor set; 
and 3) the optimal tree cover is to select the incoming edge of the maximal weight for each vertex $v$. 
This is basically the maximal spanning tree of the DAG based on the weight assignment~\cite{DBLP:conf/sigmod/JinXRW08}.
Algorithm~\ref{alg:opttreecover} sketches the optimal tree discovering procedure. 
Note that here we assume that all vertices without predecessors are connected to a virtual root.  
\input{Figures/OptimalTreeCover.tex}

To see why this method can produce the optimal index size, let us look at how a spanning tree $T$ of a DAG $G$ can compress its transitive closure. 
Given a tree $T$, the transitive closure for each vertex $u$ ($u$'s successor) of $G$ can be organized into pair-wise disjoint subtrees, and then each subtree can be represented by only its root vertex. 
In other words, the {\em compressed transitive closure} $TC_c$ of $u$ records only those vertices which $u$ can reach but without any of their corresponding ancestors in the tree (Figure~\ref{}). 
Further, let us define the total weight of the tree $T=(V,E_T)$, $W(T)=\sum_{(v^\prime,v) \in E_T} w_e = \sum_{(v^\prime,v) \in E_T} |pred(v^\prime)|$. 
Thus, a fundamental lemma is as follows: 

\blemma~\cite{SIGMOD:AgrawalBJ:1989,DBLP:conf/sigmod/JinXRW08}
For any spanning tree $T$ of DAG $G$, the size of the compressed transitive closure ($|TC_c|$) is equal to the size of the complete transitive closure ($|TC|$) minus the total weight of $T$, $W(T)$: $|TC_c|=|TC|-W(T)$. 
\elemma 

This lemma is based on the observation that if any vertex $v$ has an immediate predecessor $v^\prime$ in the tree, then the predecessors of $v^\prime$ $(pred(v^\prime))$ will not record $v$ in their compressed transitive closure. 
However, all the predecessors of $v$ except those of $v^\prime$, i.e.,  $pred(v) \backslash pred(v^\prime)$, have to record $v$. 
Thus, we can see the size of the compressed transitive closure ($TC_c$) is equal to the number of those predecessors, i.e. ,
%{\small
\beqnarr
|TC_c| = \sum_{(v^\prime,v) \in E_T} |pred(v) \backslash pred(v^\prime)| ~~~~(pred(v^\prime) \subseteq pred(v)) \nonumber \\
  =  \sum_{(v^\prime,v) \in E_T} |pred(v)| - \sum_{(v^\prime,v) \in E_T} |pred(v^\prime)| =  |TC| - W(T) \nonumber 
\eeqnarr
%}
Given this,  we can see that {\em the maximal weighted spanning tree of $G$ can minimize the size of the compressed transitive closure $TC_c$}.  

As we mentioned earlier, even though the compressed transitive closure is much smaller than $|TC|$, in order to discover the optimal tree cover,  the construction procedure needs to first compute the complete predecessor sets $TC$ (Step $1$ in Algorithm~\ref{alg:opttreecover}). 
Thus, the high computational cost $O(nm)$ and memory cost $O(n^2)$ of  the full transitive closure computation for very large graphs easily becomes the major scalability bottleneck of the tree-based reachability indexing methods. 
Note that a simple modification to reduce the memory cost is to drop the predecessor set of a vertex $v^\prime$ once all the predecessors of its immediate successors in $G$ has been computed and we only needs to record it cardinality $|pred(v^\prime)|$ instead.
However, such solution does not reduce the computational cost and its memory cost can still be too large to be scalable. 




==> abstract.tex <==
\begin{abstract}
The mean occupancy rates of personal vehicle trips in the United States is only 1.6 persons per vehicle mile. Urban traffic gridlock is a familiar scene. Ridesharing has the potential to solve many environmental, congestion, and energy problems. In this paper, we introduce the problem of large scale real-time ridesharing with service guarantee on road networks. Servers and trip requests are dynamically matched while waiting time and service time constraints of trips are satisfied. We first propose two basic algorithms: a branch-and-bound algorithm and an integer programing algorithm. However, these algorithm structures do not adapt well to the dynamic nature of the ridesharing problem. Thus, we then propose a kinetic tree algorithm capable of better scheduling dynamic requests and adjusting routes on-the-fly. We perform experiments on a large real taxi dataset from Shanghai. The results show that the kinetic tree algorithm is faster than other algorithms in response time.
\end{abstract}

